A "Game of Like" : Online Social Network Sharing As Strategic Interaction

We argue that behavioral science models of online content-sharing overlook the role of strategic interactions between users. Borrowing from accuracy-nudges studies decision-theoretic models, we propose a basic game model and explore special cases with idealized parameter settings to identify refinements necessary to capture real-world online social network behavior. Anticipating those refinements, we sketch a strategic analysis of content amplification and draw a connection between Keynes's beauty contest analogy and recent social-epistemological work on echo chambers. We conclude on the model's prospects from analytical and empirical perspectives.

==> eptcsdata.tex <==
\providecommand{\firstpage}{299}
\providecommand{\publicationstatus}{R. Verbrugge (Ed.): Theoretical Aspects of \\
Rationality and Knowledge 2023 (TARK 2023)\\
EPTCS 379, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.379.24}{10.4204/EPTCS.379.24}}

